Triplet Synthesis For Enhancing Composed Image Retrieval via Counterfactual Image Generation

Composed Image Retrieval (CIR) provides an effective way to manage and access large-scale visual data. Construction of the CIR model utilizes triplets that consist of a reference image, modification text describing desired changes, and a target image that reflects these changes. For effectively training CIR models, extensive manual annotation to construct high-quality training datasets, which can be time-consuming and labor-intensive, is required. To deal with this problem, this paper proposes a novel triplet synthesis method by leveraging counterfactual image generation. By controlling visual feature modifications via counterfactual image generation, our approach automatically generates diverse training triplets without any manual intervention. This approach facilitates the creation of larger and more expressive datasets, leading to the improvement of CIR model's performance.

==> Archive.tex <==
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{images/ICASSP1.png}
%     \vspace{-7mm}
%     \label{fig:1}
%     \setlength{\abovecaptionskip}{-5mm} % 図キャプション上空行幅調整
%     \setlength{\belowcaptionskip}{-3mm} % 図キャプション下空行幅調整
%     \caption{Examples of captioning results of multi-view lifelogging images taken in the same scene. The different captions are generated by CoCa~\cite{yu2022coca}.}
%     \vspace{-6mm}
% \end{figure}

% \begin{itemize}
%  \item 箇条書き
%  \item 箇条書き
% \end{itemize}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{images/ICASSP2_1.png}
%     \setlength{\abovecaptionskip}{-5mm} % 図キャプション上空行幅調整
%     \setlength{\belowcaptionskip}{0mm} % 図キャプション下空行幅調整
%     \caption{An overview of the proposed method.\label{fig:2}}
% \end{figure}

==> Introduction_archive.tex <==
% ================= 導入部 はじまり =================
\section{Introduction}
% \label{sec:intro}
In the digital age, the challenge of efficiently accessing and managing this vast amount of information has become more pressing.
Among the various domains impacted by this challenge, image retrieval stands out as a key field that aims to simulate and understand visual experiences similar to human perception. 
Traditional image retrieval methods~\cite{el2021training,song2023boosting} solely rely on images as input, which limits their effectiveness in handling complex queries that require both visual and contextual understanding. 
These methods often struggle to distinguish visually similar items with distinct attributes. 
They also have difficulty adapting to specific user modifications, which restricts their use in scenarios that need more precise and flexible retrievals.
To address these limitations, Composed Image Retrieval (CIR)~\cite{baldrati2023zero,gu2024lincir,saito2023pic2word} has been proposed. 
CIR enhances retrieval capabilities by utilizing both images and text as inputs. 
In other words, it is possible to acquire an image that better satisfies the user by taking the image at hand and drawing modifications to the image in text.
This dual-input approach enriches retrieval results flexibly, making it particularly valuable in fashion and e-commerce fields requiring nuanced retrievals~\cite{chen2024spirit,chen2023real20m}.

CIR holds significant potential to enhance our retrieval capabilities, but many challenges remain in applying practical models in real-world applications. 
One of the most critical of these challenges is the construction of training datasets for CIR models.
Specifically, construction of the CIR models requires datasets composed of three components: a reference image, modification text, and a target image, collectively known as triplets. 
The collection of these triplets is high-cost, traditionally relying on manual annotation~\cite{Wu_2021_CVPR,liu2021image}, which makes it difficult to collect the large-scale datasets necessary for practical model training.

To deal with this issue, Ventura et al. have proposed a method~\cite{ventura23covr} to automatically collect triplets from large-scale datasets of images and these captions. 
In this method, the construction of triplets involves two phases: collecting image pairs and creating query text. 
This method~\cite{ventura23covr} collects image pairs by focusing on the differences between words in the pre-assigned captions of images and query text corresponding to those pairs.
However, there is a significant difference between image pairs selected based solely on captions and those selected by humans, which can impact the quality of the triplets and degrade their effectiveness.
Therefore, achieving high-quality, large-scale datasets remains an essential and challenging task.

% One potential solution to the above problem is to generate images with slight modifications from the original images and use these as training triplets. 
% This paper explores the potential of counterfactual image generation methods~\cite{sauer2021counterfactual,prabhu2023lance} as a valuable approach to improve the previous method. 
% Counterfactual image generation involves breaking down features of an image (such as shape, texture, and background) and independently controlling each element to create new combinations of features.
% Thus, it can generate counterfactual images that are rich in diversity.
% The counterfactual image generation method is ideal to solve the problem of collecting high-quality triplets efficiently and at scale.
In this paper, we present a groundbreaking discovery in the realm of CIR. 
Our research uncovers the significant potential of counterfactual image generation methods for advancing CIR datasets. 
Specifically, we have found that counterfactual image generation~\cite{prabhu2023lance,le2024coco,sauer2021counterfactual}—an innovative technique that allows for the controlled manipulation of visual features, such as shape, texture, and background—can revolutionize the creation of high-quality triplet datasets for CIR.
Our discovery reveals that by leveraging counterfactual image generation, we can efficiently produce diverse and high-quality triplets without the need for manual intervention. 
This method not only enhances the scalability of dataset creation but also addresses common issues such as learning spurious correlations from real images. 
Instead, it enables the model to learn features that are directly relevant to the primary subject, thereby improving the robustness of retrieval models.


% Overview図挿入
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/ICASSP_figure_NS_crop.pdf}
    \vspace{-5mm}
    \setlength{\abovecaptionskip}{0mm} % 図キャプション上空行幅調整
    \setlength{\belowcaptionskip}{0mm} % 図キャプション下空行幅調整
    \caption{\textbf{Overview of the Proposed Triplet Generation Method.}
    This figure shows the process of generating triplets to improve CIR performance. It involves modifying the reference caption $c_{\rm{ref}}$ to create a counterfactual caption $c_{\rm{cf}}$ and generating a corresponding image. These triplets enhance the diversity of training data for CIR models.\label{fig:overview}}
    \vspace{-3mm}
\end{figure*}

% This breakthrough provides a new, efficient approach for generating training data, setting a precedent for future research and practical applications in CIR. The implications of this discovery are substantial, offering a novel solution to longstanding challenges in automatic triplet generation and laying the groundwork for more advanced and effective CIR systems.

Therefore, we propose data augmentation for CIR datasets using counterfactual image generation models. 
The proposed method enables the creation of high-quality triplet datasets based on slight modifications without manual annotation. 
Additionally, learning from real images may lead to learning spurious correlations—relationships that appear in data but are not directly relevant. 
Counterfactual image generation allows learning features that are more directly related to the main subject. 
A deeper comprehension of these relationships can enhance the robustness of retrieval models. 
Consequently, using counterfactual image generation models can overcome traditional challenges in automatic triplet generation for CIR and facilitate the creation of practical, large-scale CIR datasets.
This paper investigates the use of datasets generated by counterfactual image generation models to CIR. 
We demonstrate how the proposed method can improve CIR model performance by providing a scalable and efficient method for generating the necessary training data.
In summary, the contributions of this paper are shown as follows.

\begin{itemize}
  \item  Implementing a data augmentation method for CIR through counterfactual image generation models, thereby enhancing the quality and diversity of training datasets.

  \item Enhancing CIR model performance through a scalable and efficient data generation method using counterfactual image generation.
\end{itemize}
These contributions offer new insights and practical solutions for CIR, laying a solid foundation for future research and implementation.

% ================= 導入部 おわり =================

==> tables/ablation_dataset_scale.tex <==
\begin{table}[t!]
    \caption{\small Ablation study on the introduction of a counterfactual check mechanism}
    \vspace{2mm}
    \centering
    \small % フォントサイズを小さくする
    \begin{tabular}{llcccc}
        \toprule[1.0pt]
        \multirow{2}{*}{Methods} & \multirow{2}{*}{Data} & \multicolumn{4}{c}{Counterfactual data scale} \\
        \cmidrule(lr){3-6}
        & & 100 & 500 & 1000 & 10000 \\
        \midrule[0.05em]
        TIRG (Vo '19) & - &  &  &  &  \\
        TRACE & - & - & - &  &  \\
        CompoDiff & ST18M &  &  &  &  \\
        \bottomrule[1.0pt]
    \end{tabular}
    \label{tab:data_statistics}
    \vspace{-3mm}
\end{table}



==> tables/counterfactual_check.tex <==
% Modification text の生成方法
\begin{table}[t!] 
    \caption{\small Results of comparison with modification text generation methods.}
    \vspace{2mm}
    \centering
    {
    \begin{tabular}{l|cc|cc}
        \toprule
        & \multicolumn{2}{c|}{FashionIQ}  & \multicolumn{2}{c}{CIRR}\\
        Model & R@1 & MeanR & R@1 & MeanR \\ 
        \midrule
        LANCE & & & & \\
        Rule-based &  &  & &  \\
        % \rowcolor{green!15}
        LLaMA-3.1-8B & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:counterfactual check}
    \vspace{-3mm}
\end{table}

==> tables/main_result_archive.tex <==
% 掲載する実験結果
\begin{table*}[ht!]
    \caption{\textbf{Experimental Results on CIRR (Test Data) and FashionIQ (Validation Data).}
    This table compares the performance of various models on reduced image sets (30\% of the original number of images for both FashionIQ and CIRR). 
    The table includes results for zero-shot learning, previous methods without counterfactual data, and our proposed method that incorporates counterfactual data for training. 
    Performance metrics are reported in terms of Recall at different ranks (R@1, R@5, R@10, R@50), showing how our counterfactual data augmentation approach enhances model performance.}
    \vspace{2mm}
    \centering
    \small % フォントサイズを小さくする
    \begin{tabular}{lllcccccccc}
        \toprule[1.0pt]
        \multirow{2}{*}{Mode} & \multirow{2}{*}{Methods} & \multirow{2}{*}{Pretraining Data} & \multicolumn{4}{c}{CIRR} & \multicolumn{2}{c}{FashionIQ} \\
        \cmidrule(lr){4-7} \cmidrule(lr){8-9} 
        & & & R@1 & R@5 & R@10 & R@50 & R@10 & R@50 \\
        \midrule[0.05em]
        \multirow{3}{*}{Zero Shot} & Pic2Word (Saito '23) & CC3M & 23.90 & 51.70 & 65.30 & 87.80 & 24.70 & 43.70 \\
                                   & CompoDiff (Gu '23) & ST18M &19.37 &53.81 &72.02 &90.85 &35.62 &48.45 \\
                                   % & CASE (Levy '23) & LaSCo &30.89 &60.75  &73.88 &92.84 &  &  \\
                                   % & CASE (Levy '23) & LaSCo+COCO &35.40 &65.78 & 78.53 & 94.63 &  &  \\
                                   & SEARLE (Baldrati '23) &-  & & & & & & \\
                                   % & CoVR-BLIP &- &39.28 &68.22 &78.94 &94.65 &27.70 &44.63 \\
        \midrule[0.05em]
        \multicolumn{9}{c}{Previous methods (without counterfactual data)}  \\
        \midrule[0.05em]
        \multirow{3}{*}{Train} &ARTEMIS (Delmas '22) &- &5.59 &18.05 &27.57 &57.11 &&\\%& ARTEMIS &- &19.37 &53.81 &72.02 &90.85 & & \\
                               & Combiner (Baldrati '23) &- &32.65 &63.78 &75.59 &93.28 &31.93 &54.62 \\
                               & CoVR-BLIP (Ventura '24)  &- &39.66 &68.07 &78.17 &93.01 &36.34 &58.27 \\
        \midrule[0.05em]
        \multicolumn{9}{c}{Results with the models trained with counterfactual data}  \\
        \midrule[0.05em]
        \multirow{3}{*}{Train (Ours)} &ARTEMIS (Delmas '22) &- &3.78&12.60&21.66&50.17&&\\%& ARTEMIS &- &18.76 &49.29 &64.37 &89.36 & & \\
                               & Combiner (Baldrati '23) &- &32.58 &63.78 &75.60 &94.12 &&&\\%42.58 &65.81 \\
                               & CoVR-BLIP (Ventura '24) &- &\textbf{40.75} &\textbf{69.83} &\textbf{81.04} &\textbf{94.80} &\textbf{39.13} &\textbf{60.61} \\
        \bottomrule[1.0pt]
    \end{tabular}
    \label{tab:results_1}
\end{table*}
